Hybrid Beamforming for Millimeter Wave Full-Duplex under Limited Receive Dynamic Range

Full-duplex millimeter wave (mmWave) communication has shown increasing promise for self-interference cancellation via hybrid precoding and combining. This paper proposes a novel mmWave multiple-input multiple-output (MIMO) design for configuring the analog and digital beamformers of a full-duplex transceiver. Our design is the first to holistically consider the key practical constraints of analog beamforming codebooks, a minimal number of radio frequency (RF) chains, limited channel knowledge, beam alignment, and a limited receive dynamic range. To prevent self-interference from saturating the receiver of a full-duplex device having limited dynamic range, our design addresses saturation on a per-antenna and per-RF chain basis. Numerical results evaluate our design in a variety of settings and validate the need to prevent receiver-side saturation. These results and the corresponding insights serve as useful design references for practical full-duplex mmWave transceivers.

==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/

For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


***************************** Subdirectories ******************************

bibtex   - The IEEEtran BibTeX style package.

extras   - Supplementary material that may be of interest.

testflow - The testflow diagnostic suite for verifying PS/PDF output.

tools    - The IEEEtrantools.sty package which provides several commands
           from the IEEEtran.cls file for use with other LaTeX classes.


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf.tex          - A bare bones starter file for IEEE conference papers.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl.tex          - A bare bones starter file for IEEE journal papers.

bare_jrnl_comsoc.tex   - A bare bones starter file for IEEE Communications
                         Society journal papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_jrnl_transmag.tex - A bare bones starter file for IEEE Transactions
                         on Magnetics journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for an IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf.tex, bare_conf_compsoc.tex,
                   bare_jrnl.tex, bare_jrnl_comsoc.tex,
                   bare_jrnl_compsoc.tex, bare_jrnl_transmag.tex
***************************************************************************


==> alg/algorithm-v1.tex <==
\begin{figure}[!ht]
	\begin{algorithmic}[0]
		\REQUIRE knowledge of $\rho_{ij}, \Ns\node{i}, \comrf\node{j}, \prerf\node{i}, \comrf\ctransnode{j} \channel_{ij} \prerf\node{i}, \Ptxwatts\node{i}, G_{ii}, \channel_{ii}, \comrf\node{i}, \powersimaxlna, \powersimaxadc$
		\REQUIRE $\nu_{\mathrm{min}}$, $\nu_{\mathrm{max}}$, $N_{\nu}$, $\epspow$, $\epslna$, $\epsadc$, initial choice of $\prebb\node{i}$ 
		\STATE $\nu \leftarrow \nu_{\mathrm{max}}$
		\REPEAT
			\STATE Solve \eqref{eq:unconstrained-augmented-2} for $\prebb\node{i}$ using the Adam algorithm.
			\STATE Compute $\mathcal{I}_{ij}\parens{\prebb\node{i}}$, $\mathcal{C}_{\mathrm{pow}}\parens{\prebb\node{i}}$,
			$\mathcal{C}_{\mathrm{LNA}}\parens{\prebb\node{i}}$, and 
			$\mathcal{C}_{\mathrm{ADC}}\parens{\prebb\node{i}}$.
			\IF{$\mathcal{C}_{\mathrm{pow}}\parens{\prebb\node{i}} \leq \epsilon_{\mathrm{pow}}$ and	$\mathcal{C}_{\mathrm{LNA}}\parens{\prebb\node{i}}  \leq \epslna \cdot \powersimaxlna$ and
				$\mathcal{C}_{\mathrm{ADC}}\parens{\prebb\node{i}}  \leq \epsadc \cdot \powersimaxadc$}
				\IF{$\mathcal{I}_{ij}\parens{\prebb\node{i}} \geq \mathcal{I}_{ij}\opt$}
					\STATE $\mathcal{I}_{ij}\opt \leftarrow \mathcal{I}_{ij}\parens{\prebb\node{i}}$
					\STATE ${\prebb\node{i}}\opt \leftarrow \prebb\node{i}$
				\ENDIF
				\STATE $\nu_{\mathrm{max}} \leftarrow \nu$ \quad \textit{(relax constraints, decrease $\nu$)}
			\ELSE
				\STATE $\nu_{\mathrm{min}} \leftarrow \nu$ \quad \textit{(enforce constraints, increase $\nu$)}
			\ENDIF
			\STATE $\nu \leftarrow \parens{\nu_{\mathrm{min}} + \nu_{\mathrm{max}}} / 2$
		\UNTIL{maximum number of bisection steps reached or sufficiently close to achieving capacity}
		\STATE ${\prebb\node{i}} \leftarrow {\prebb\node{i}}\opt$
		\IF{$\frobeniustwo{\prebb\node{i}} > 1$}
		\STATE $\prebb\node{i} \leftarrow \prebb\node{i}  \ / \ \frobenius{\prebb\node{i}}$ \quad \textit{(transmit power projection)}
		\ENDIF
		\IF{$\frac{1}{\Ns\node{i}} \norminf{\sqrt{\Ptxwatts\node{i}} G_{ii} \channel_{ii} \prerf\node{i} \prebb\node{i}}^2 > \powersimaxlna$}
		\STATE $\prebb\node{i} \leftarrow \prebb\node{i}  \ \times \sqrt{\powersimaxlna} \ / \ \frac{1}{\sqrt{\Ns\node{i}}} \norminf{\sqrt{\Ptxwatts\node{i}} G_{ii} \channel_{ii} \prerf\node{i} \prebb\node{i}}$ \quad \textit{(LNA power projection)}
		\ENDIF
		\IF{$\frac{1}{\Ns\node{i}} \norminf{\sqrt{\Ptxwatts\node{i}} G_{ii} \comrf\ctransnode{i} \channel_{ii} \prerf\node{i} \prebb\node{i}}^2 > \powersimaxadc$}
		\STATE $\prebb\node{i} \leftarrow \prebb\node{i}  \ \times \sqrt{\powersimaxadc} \ / \ \frac{1}{\sqrt{\Ns\node{i}}} \norminf{\sqrt{\Ptxwatts\node{i}} G_{ii} \comrf\ctransnode{i} \channel_{ii} \prerf\node{i} \prebb\node{i}}$ \quad \textit{(ADC power projection)}
		\ENDIF
	\end{algorithmic}
	\caption{Our algorithm for solving \eqref{eq:problem-inner}.}
\end{figure}

==> mathtype.tex <==
\usepackage{bm}

% Vectors
\def\vzero{{\vec{0}}}
\def\vone{{\vec{1}}}
\def\vmu{{\vec{\mu}}}
\def\vtheta{{\vec{\theta}}}
\def\va{{\vec{a}}}
\def\vb{{\vec{b}}}
\def\vc{{\vec{c}}}
\def\vd{{\vec{d}}}
\def\ve{{\vec{e}}}
\def\vf{{\vec{f}}}
\def\vg{{\vec{g}}}
\def\vh{{\vec{h}}}
\def\vi{{\vec{i}}}
\def\vj{{\vec{j}}}
\def\vk{{\vec{k}}}
\def\vl{{\vec{l}}}
\def\vm{{\vec{m}}}
\def\vn{{\vec{n}}}
\def\vo{{\vec{o}}}
\def\vp{{\vec{p}}}
\def\vq{{\vec{q}}}
\def\vr{{\vec{r}}}
\def\vs{{\vec{s}}}
\def\vt{{\vec{t}}}
\def\vu{{\vec{u}}}
\def\vv{{\vec{v}}}
\def\vw{{\vec{w}}}
\def\vx{{\vec{x}}}
\def\vy{{\vec{y}}}
\def\vz{{\vec{z}}}

% Matrix
\def\mA{{\mat{A}}}
\def\mB{{\mat{B}}}
\def\mC{{\mat{C}}}
\def\mD{{\mat{D}}}
\def\mE{{\mat{E}}}
\def\mF{{\mat{F}}}
\def\mG{{\mat{G}}}
\def\mH{{\mat{H}}}
\def\mI{{\mat{I}}}
\def\mJ{{\mat{J}}}
\def\mK{{\mat{K}}}
\def\mL{{\mat{L}}}
\def\mM{{\mat{M}}}
\def\mN{{\mat{N}}}
\def\mO{{\mat{O}}}
\def\mP{{\mat{P}}}
\def\mQ{{\mat{Q}}}
\def\mR{{\mat{R}}}
\def\mS{{\mat{S}}}
\def\mT{{\mat{T}}}
\def\mU{{\mat{U}}}
\def\mV{{\mat{V}}}
\def\mW{{\mat{W}}}
\def\mX{{\mat{X}}}
\def\mY{{\mat{Y}}}
\def\mZ{{\mat{Z}}}
\def\mBeta{{\mat{\beta}}}
\def\mPhi{{\mat{\Phi}}}
\def\mLambda{{\mat{\Lambda}}}
\def\mSigma{{\mat{\Sigma}}}

==> mymath.tex <==
% COMMENT OUT
\newcommand{\comment}[1]{{}}

% TEXT
\usepackage{amssymb}
\usepackage{xspace}
\newcommand{\super}[1]{\textsuperscript{#1}\xspace}

% COMPLEX & NUMBERS
\newcommand{\real}{\ensuremath{\mathbb{R}}\xspace}
\newcommand{\realpow}[2]{\ensuremath{\real^{#1 \times #2}}\xspace}
\newcommand{\complex}{\ensuremath{\mathbb{C}}\xspace}
\newcommand{\complexpow}[2]{\ensuremath{\complex^{#1 \times #2}}\xspace}
\newcommand{\conj}{\ensuremath{^{*}}\xspace}
\renewcommand{\j}{\ensuremath{\mathrm{j}}}
\newcommand{\todB}[1]{\ensuremath{\entry{#1}{\mathrm{dB}}}}
\newcommand{\todBm}[1]{\ensuremath{\entry{#1}{\mathrm{dBm}}}}

\usepackage{bm}

\newcommand{\Ts}{\ensuremath{T_{\textrm{s}}}}
\newcommand{\fs}{\ensuremath{f_{\textrm{s}}}}
\newcommand{\cplength}{\ensuremath{N_{\textrm{CP}}}}

% LINEAR ALGEBRA
\newcommand{\inv}{\ensuremath{^{-1}}\xspace}
\newcommand{\trans}{\ensuremath{^{\textsf{T}}}\xspace}
\newcommand{\ctrans}{\ensuremath{^{{*}}}\xspace}
\newcommand{\opt}{\ensuremath{^{{\star}}}\xspace}
\newcommand{\mat}[1]{\ensuremath{\mathbf{#1}}\xspace} % matrices
\renewcommand{\vec}[1]{\ensuremath{\mathbf{#1}}\xspace} % vectors
\newcommand{\matfd}[1]{\ensuremath{\bm{\mathsf{#1}}}\xspace} % matrices in frequency domain
\newcommand{\vecfd}[1]{\ensuremath{\bm{\mathsf{#1}}}\xspace} % vectors in frequency domain
\newcommand{\zerovec}{\ensuremath{\vec{0}}\xspace}
\newcommand{\eyevec}[1]{\ensuremath{\vec{1}_{#1}}\xspace}
\newcommand{\eyemat}[1]{\ensuremath{\mat{I}_{#1}}\xspace}
\newcommand{\zeromat}{\ensuremath{\mat{0}}\xspace}
\newcommand{\trace}{\ensuremath{\mathrm{tr}}}
\newcommand{\norm}[1]{\left\lVert#1\right\rVert}
\newcommand{\card}[1]{\left\lvert#1\right\rvert}
\newcommand{\pnorm}[2]{\ensuremath{\left\lVert{#2}\right\rVert_{#1}}\xspace}
\newcommand{\pinv}[1]{\left({#1\ctrans} {#1}\right)^{-1}{#1\ctrans}}

\newcommand{\entry}[2]{\ensuremath{\left[{#1}\right]_{#2}}\xspace}

\newcommand{\rank}[1]{\ensuremath{\textrm{rank}\left({#1}\right)}}
\newcommand{\col}[1]{\ensuremath{\textrm{col}\left({#1}\right)}\xspace}

\newcommand{\myspan}{\ensuremath{\mathrm{span}}}
\newcommand{\st}{\ensuremath{\mathrm{s.t.~}}}

\newcommand{\svd}[1]{\ensuremath{\mat{U}_{#1} \ \mat{\Sigma}_{#1} \ \mat{V}\ctrans_{#1} }}
\newcommand{\svdfd}[2]{\ensuremath{\matfd{U}_{#1}#2 \ \matfd{\Sigma}_{#1}#2 \ \matfd{V}\ctrans_{#1}#2 }}

\newcommand{\sing}[1]{\ensuremath{\mat{\Sigma}_{#1} }}
\newcommand{\lsing}[1]{\ensuremath{\mat{U}_{#1} }}
\newcommand{\rsing}[1]{\ensuremath{\mat{V}_{#1} }}

\newcommand{\singfd}[2]{\ensuremath{\matfd{\Sigma}_{#1}#2 }}
\newcommand{\lsingfd}[2]{\ensuremath{\matfd{U}_{#1}#2 }}
\newcommand{\rsingfd}[2]{\ensuremath{\matfd{V}_{#1}#2 }}

% SETS
\newcommand{\set}[1]{\ensuremath{\mathcal{#1}}\xspace} % caligraphic set notation

% PROB/STATS/ANALYSIS
\newcommand{\gauss}[2]{\ensuremath{\mathcal{N} \left( #1 , #2 \right) }\xspace} % gaussian/normal distribution
\newcommand{\cgauss}[2]{\ensuremath{\mathcal{N}_{\complex} \left( {#1} , {#2} \right) }\xspace} % complex gaussian/normal distribution
\newcommand{\ev}[1]{\ensuremath{\mathbb{E}\left[{#1}\right]}\xspace}
\newcommand{\uniform}[2]{\ensuremath{\textrm{Unif}\left(#1,#2\right)}}
\newcommand{\exponential}[1]{\ensuremath{\textrm{Exp}\left(#1\right)}}
\newcommand{\laplace}[2]{\ensuremath{\textrm{Laplace}\left(#1,#2\right)}}

% MIMO
\newcommand{\pre}{\ensuremath{\mat{F}}\xspace} 				   % precoder
\newcommand{\prebb}{\ensuremath{\mat{F}_{\mathrm{BB}}}\xspace} % baseband precoder
\newcommand{\prebbfd}{\ensuremath{\matfd{F}_{\mathsf{BB}}}\xspace} % baseband precoder
\newcommand{\prerffd}{\ensuremath{\matfd{F}_{\mathsf{RF}}}\xspace} % baseband precoder
\newcommand{\prebbfdtilde}{\ensuremath{\hat{\matfd{F}}_{\mathsf{BB}}}\xspace} % baseband precoder

\newcommand{\prefd}{\ensuremath{\matfd{F}}\xspace} % baseband precoder
\newcommand{\prerf}{\ensuremath{\mat{F}_{\mathrm{RF}}}\xspace} % RF precoder
\newcommand{\com}{\ensuremath{\mat{W}}\xspace} 				   % combiner
\newcommand{\combb}{\ensuremath{\mat{W}_{\mathrm{BB}}}\xspace} % baseband combiner
\newcommand{\combbfd}{\ensuremath{\matfd{W}_{\mathsf{BB}}}\xspace} % baseband combiner
\newcommand{\comfd}{\ensuremath{\matfd{W}}\xspace} % baseband precoder
\newcommand{\combbfdtrans}{\ensuremath{\tilde{\matfd{W}}_{\textrm{BB}}}\xspace} % baseband combiner
\newcommand{\comrf}{\ensuremath{\mat{W}_{\mathrm{RF}}}\xspace} % RF combiner
\newcommand{\comrffd}{\ensuremath{\matfd{W}_{\mathsf{RF}}}\xspace} % RF combiner

\newcommand{\xbb}{\ensuremath{\mat{X}_{\mathrm{BB}}}\xspace} % baseband beamformer
\newcommand{\xrf}{\ensuremath{\mat{X}_{\mathrm{RF}}}\xspace} % RF beamformer

\newcommand{\xfd}{\ensuremath{\matfd{X}}\xspace} % baseband beamformer
\newcommand{\xbbfd}{\ensuremath{\matfd{X}_{\mathsf{BB}}}\xspace} % baseband beamformer
\newcommand{\xrffd}{\ensuremath{\matfd{X}_{\mathsf{RF}}}\xspace} % RF beamformer
\newcommand{\xbbfdtilde}{\ensuremath{\bar{\matfd{X}}_{\mathsf{BB}}}\xspace} % baseband precoder

\newcommand{\precb}{\ensuremath{\mathcal{F}_{\mathrm{RF}}}\xspace}
\newcommand{\prebbcb}{\ensuremath{\mathcal{F}_{\mathrm{BB}}}\xspace}

%\newcommand{\prerfcb}{\ensuremath{\mathcal{F}_{\mathrm{RF}}}\xspace}
%\newcommand{\comrfcb}{\ensuremath{\mathcal{W}_{\mathrm{RF}}}\xspace}
\newcommand{\prerfcb}{\ensuremath{\mathcal{F}}\xspace}
\newcommand{\comrfcb}{\ensuremath{\mathcal{W}}\xspace}

%\newcommand{\prerfcbcand}{\ensuremath{\tilde{\mathcal{F}}_{\mathrm{RF}}}\xspace}
%\newcommand{\comrfcbcand}{\ensuremath{\tilde{\mathcal{W}}_{\mathrm{RF}}}\xspace}
\newcommand{\prerfcbcand}{\ensuremath{\tilde{\mathcal{F}}}\xspace}
\newcommand{\comrfcbcand}{\ensuremath{\tilde{\mathcal{W}}}\xspace}

\newcommand{\numprerfcbcand}{\ensuremath{K_{\mathrm{pre}}}\xspace}
\newcommand{\numcomrfcbcand}{\ensuremath{K_{\mathrm{com}}}\xspace}

\newcommand{\precbmat}{\ensuremath{\mat{A}_{\mathsf{RF}}}\xspace}
\newcommand{\Arffd}{\ensuremath{\matfd{A}_{\mathsf{RF}}}\xspace}
\newcommand{\tildeprecbmat}{\ensuremath{\tilde{\mat{A}}_{\mathsf{RF}}}\xspace}

\newcommand{\channel}{\ensuremath{\mat{H}}\xspace} % MIMO channel
\newcommand{\channeltilde}{\ensuremath{\tilde{\mat{H}}}\xspace} % MIMO channel
\newcommand{\channeltildedelta}{\ensuremath{\Delta\tilde{\mat{H}}}\xspace} % MIMO channel
\newcommand{\channeltildebar}{\ensuremath{\hat{\tilde{\mat{H}}}}\xspace} % MIMO channel
\newcommand{\channelfd}{\ensuremath{\matfd{H}}\xspace} % MIMO channel
\newcommand{\noisevar}{\ensuremath{\sigma^2_{\mathrm{n}}}\xspace}

\newcommand{\channeldes}{\ensuremath{\channel_{\mathrm{des}}}\xspace}
\newcommand{\channelint}{\ensuremath{\channel_{\mathrm{int}}}\xspace}

\newcommand{\symbveccb}{\ensuremath{\mathcal{S}}\xspace}

\newcommand{\Nt}{\ensuremath{N_\mathrm{t}}\xspace} % number of antennas at Tx
\newcommand{\Nr}{\ensuremath{N_\mathrm{r}}\xspace} % number of antennas at Rx
\newcommand{\Na}{\ensuremath{N_{\mathrm{a}}}\xspace} % number of antennas

\newcommand{\Nrf}{\ensuremath{N_\mathrm{RF}}\xspace} % number of RF chains
\newcommand{\Nrftx}{\ensuremath{L_{\mathrm{t}}}\xspace} % number of RF chains at Tx
\newcommand{\Nrfrx}{\ensuremath{L_{\mathrm{r}}}\xspace} % number of RF chains at Rx
% \newcommand{\Nrfrx}{\ensuremath{{\Nrf}_{\textrm{r}}}\xspace} % number of RF chains at Rx

\newcommand{\Ns}{\ensuremath{N_\mathrm{s}}\xspace} % number of spatial streams
%\newcommand{\Nstx}{\ensuremath{\Ns^\textrm{t}}\xspace} % number of spatial streams at Tx
\newcommand{\Nstx}{\ensuremath{N_\textrm{s,tx}}\xspace} % number of spatial streams at Tx
\newcommand{\Nsrx}{\ensuremath{N_\textrm{s,rx}}\xspace} % number of spatial streams at Rx
%\newcommand{\Nsrx}{\ensuremath{\Ns^\textrm{r}}\xspace} % number of spatial streams at Rx

\newcommand{\Rs}{\ensuremath{\mat{R}_{\mathrm{s}}\xspace}}
\newcommand{\Rn}{\ensuremath{\mat{R}_{\mathrm{n}}\xspace}}
\newcommand{\Rsfd}{\ensuremath{\matfd{R}_{\mathsf{s}}\xspace}}
\newcommand{\Rnfd}{\ensuremath{\matfd{R}_{\mathsf{n}}\xspace}}

\newcommand{\Pt}{\ensuremath{P_{\mathrm{tx}}\xspace}}

\newcommand{\symbvec}{\ensuremath{\vec{s}}\xspace}
\newcommand{\noisevec}{\ensuremath{\vec{n}}\xspace}
\newcommand{\rxvec}{\ensuremath{\hat{\vec{s}}}\xspace}

\newcommand{\symbvecfd}{\ensuremath{\vecfd{s}}\xspace}
\newcommand{\noisevecfd}{\ensuremath{\vecfd{n}}\xspace}
\newcommand{\rxvecfd}{\ensuremath{\hat{\vecfd{s}}}\xspace}

\newcommand{\rxsi}{\ensuremath{\vec{y}_{\textrm{SI}}}\xspace}
\newcommand{\rxsiest}{\ensuremath{\hat{\vec{y}}_{\textrm{SI}}}\xspace}
\newcommand{\rxout}{\ensuremath{\vec{y}_{\textrm{out}}}\xspace}

% RAY/CLUSTER MODEL
\newcommand{\numrays}{\ensuremath{N_{\mathrm{rays}}}\xspace}
\newcommand{\numclust}{\ensuremath{N_{\mathrm{clust}}}\xspace}

% SI CHANNEL
\newcommand{\sichannel}{\ensuremath{\mat{H}_{\textrm{SI}}}\xspace}
\newcommand{\sichannellos}{\ensuremath{\mat{H}_{\textrm{SI,LOS}}}\xspace}
\newcommand{\sichannelnlos}{\ensuremath{\mat{H}_{\textrm{SI,NLOS}}}\xspace}

% RICEAN
\newcommand{\ricefactor}{\ensuremath{\kappa}\xspace}
\newcommand{\ricelos}{\ensuremath{\sqrt{\frac{\ricefactor}{\ricefactor + 1}}}\xspace}
\newcommand{\ricenlos}{\ensuremath{\sqrt{\frac{1}{\ricefactor + 1}}}\xspace}

% NORMS
\newcommand{\frobenius}[1]{\ensuremath{\pnorm{\mathrm{F}}{#1}}}
\newcommand{\frobeniustwo}[1]{\ensuremath{\left\Vert#1\right\Vert^{2}_{\mathrm{F}}}}

% fix this
\newcommand{\azimuth}{\ensuremath{\theta}\xspace}
\newcommand{\elevation}{\ensuremath{\phi}\xspace}
\newcommand{\aoa}{\ensuremath{\Theta}\xspace}
\newcommand{\aod}{\ensuremath{\Phi}\xspace}

\newcommand{\rxresponsevector}{\ensuremath{\vec{a}_{\mathrm{r}}(\azimuth_{i,j},\elevation_{i,j})}\xspace}
\newcommand{\txresponsevector}{\ensuremath{\vec{a}_{\mathrm{t}}(\azimuth_{i,j},\elevation_{i,j})}\xspace}

\renewcommand{\rxresponsevector}{\ensuremath{\vec{a}_{\mathrm{r}}}\xspace}
\renewcommand{\txresponsevector}{\ensuremath{\vec{a}_{\mathrm{t}}}\xspace}

% MISC
\newcommand{\enob}{\ensuremath{\mathcal{E}}\xspace}
\newcommand{\snr}{\ensuremath{\mathrm{SNR}}\xspace}
\newcommand{\sqnr}{\ensuremath{\mathrm{SQNR}}\xspace}
\newcommand{\sqr}{\ensuremath{\mathrm{SQR}}\xspace}
\newcommand{\qnr}{\ensuremath{\mathrm{QNR}}\xspace}
\newcommand{\sinr}{\ensuremath{\mathrm{SINR}}\xspace}
\newcommand{\sir}{\ensuremath{\mathrm{SIR}}\xspace}
\newcommand{\inr}{\ensuremath{\mathrm{INR}}\xspace}
 
% TRADEOFF STUFF
\newcommand{\fdsnr}{\ensuremath{\tilde{\snr}}}
\newcommand{\fdsinr}{\ensuremath{\tilde{\sinr}}}
\newcommand{\fdsir}{\ensuremath{\tilde{\sir}}}
\newcommand{\fdinr}{\ensuremath{\tilde{\inr}}}

\newcommand{\fdulsnr}[1]{\ensuremath{\tilde{\snr}^{\textrm{UL}}_{#1}}}
\newcommand{\fdulsinr}[1]{\ensuremath{\tilde{\sinr}^{\textrm{UL}}_{#1}}}
\newcommand{\fdulsir}[1]{\ensuremath{\tilde{\sir}^{\textrm{UL}}_{#1}}}
\newcommand{\fdulinr}[1]{\ensuremath{\tilde{\inr}^{\textrm{UL}}_{#1}}}

\newcommand{\fddlsnr}[1]{\ensuremath{\tilde{\snr}^{\textrm{DL}}_{#1}}}
\newcommand{\fddlsinr}[1]{\ensuremath{\tilde{\sinr}^{\textrm{DL}}_{#1}}}
\newcommand{\fddlsir}[1]{\ensuremath{\tilde{\sir}^{\textrm{DL}}_{#1}}}
\newcommand{\fddlinr}[1]{\ensuremath{\tilde{\inr}^{\textrm{DL}}_{#1}}}

\newcommand{\fdrate}{\ensuremath{\tilde{R}}}
\newcommand{\fdulrate}[1]{\ensuremath{\tilde{R}^{\textrm{UL}}_{#1}}}
\newcommand{\fddlrate}[1]{\ensuremath{\tilde{R}^{\textrm{DL}}_{#1}}}

\newcommand{\fdhdulrate}[1]{\ensuremath{\hat{R}^{\textrm{UL}}_{#1}}}
\newcommand{\fdhddlrate}[1]{\ensuremath{\hat{R}^{\textrm{DL}}_{#1}}}

\newcommand{\hdsnr}[1]{\ensuremath{{\snr}_{#1}}}
\newcommand{\hdsinr}[1]{\ensuremath{{\sinr}_{#1}}}
\newcommand{\hdsir}[1]{\ensuremath{{\sir}_{#1}}}
\newcommand{\hdinr}[1]{\ensuremath{{\inr}_{#1}}}

\newcommand{\hdulsnr}[1]{\ensuremath{{\snr}^{\textrm{UL}}_{#1}}}
\newcommand{\hdulsinr}[1]{\ensuremath{{\sinr}^{\textrm{UL}}_{#1}}}
\newcommand{\hdulsir}[1]{\ensuremath{{\sir}^{\textrm{UL}}_{#1}}}
\newcommand{\hdulinr}[1]{\ensuremath{{\inr}^{\textrm{UL}}_{#1}}}

\newcommand{\hddlsnr}[1]{\ensuremath{{\snr}^{\textrm{DL}}_{#1}}}
\newcommand{\hddlsinr}[1]{\ensuremath{{\sinr}^{\textrm{DL}}_{#1}}}
\newcommand{\hddlsir}[1]{\ensuremath{{\sir}^{\textrm{DL}}_{#1}}}
\newcommand{\hddlinr}[1]{\ensuremath{{\inr}^{\textrm{DL}}_{#1}}}

\newcommand{\hdrate}{\ensuremath{{R}}}
\newcommand{\hdulrate}[1]{\ensuremath{{R}^{\textrm{UL}}_{#1}}}
\newcommand{\hddlrate}[1]{\ensuremath{{R}^{\textrm{DL}}_{#1}}}

\newcommand{\hdulcap}[1]{\ensuremath{{C}^{\textrm{UL}}_{#1}}}
\newcommand{\hddlcap}[1]{\ensuremath{{C}^{\textrm{DL}}_{#1}}}

\newcommand{\fdulcap}[1]{\ensuremath{\tilde{C}^{\textrm{UL}}_{#1}}}
\newcommand{\fddlcap}[1]{\ensuremath{\tilde{C}^{\textrm{DL}}_{#1}}}

\newcommand{\hdcap}{\ensuremath{C}}
\newcommand{\fdcap}{\ensuremath{\tilde{C}}}

\newcommand{\ulcap}[1]{\ensuremath{{C}^{\textrm{UL}}_{#1}}}
\newcommand{\dlcap}[1]{\ensuremath{{C}^{\textrm{DL}}_{#1}}}
 
\newcommand{\degul}[1]{\ensuremath{\gamma^{\textrm{UL}}_{#1}}}
\newcommand{\degdl}[1]{\ensuremath{\gamma^{\textrm{DL}}_{#1}}}
 
% NODES
\newcommand{\anode}[2]{\ensuremath{{{#1}^{X}}^{\left(#2\right)}}\xspace}
\newcommand{\bnode}[1]{\textsuperscript{\ensuremath{(#1)}}}
\newcommand{\node}[1]{\unskip\ensuremath{^{^{\left(#1\right)}}}\xspace}

% \newcommand{\ctransnode}[1]{\ensuremath{^{{*}^{\left(#1\right)}}}\xspace}
\newcommand{\ctransnode}[1]{\ensuremath{^{^{\left(#1\right)}{*}}}\xspace}
\newcommand{\nullspace}[1]{\ensuremath{\textrm{null}\left(#1\right)}}
\newcommand{\kernel}[1]{\ensuremath{\mathrm{ker}\left(#1\right)}}

% PSEUDOCODE
\newcommand{\zeros}[1]{\ensuremath{\textrm{zeros}\left(#1\right)}}
\newcommand{\ones}[1]{\ensuremath{\textrm{ones}\left(#1\right)}}
\newcommand{\abs}[1]{\ensuremath{\textrm{abs}\left(#1\right)}}
% \newcommand{\angle}[1]{\ensuremath{\textrm{angle}\left(#1\right)}}

\newcommand{\adcfun}[2]{\ensuremath{\mathcal{Q}_{#1}\left(#2\right)}}
\newcommand{\lnafun}[1]{\ensuremath{\mathcal{L}\left(#1\right)}}
\newcommand{\lnafunlin}[1]{\ensuremath{\mathcal{L}_{\mathrm{lin}}\left(#1\right)}}
\newcommand{\lnafunsat}[1]{\ensuremath{\mathcal{L}_{\mathrm{sat}}\left(#1\right)}}

\newcommand{\ylna}{\ensuremath{\vec{y}_{\mathrm{LNA}}}\xspace}
\newcommand{\yadc}{\ensuremath{\vec{y}_{\mathrm{ADC}}}\xspace}
\newcommand{\etalna}{\ensuremath{\eta_{\mathrm{LNA}}}\xspace}
\newcommand{\etaadc}{\ensuremath{\eta_{\mathrm{ADC}}}\xspace}
\newcommand{\PonedB}{\ensuremath{\mathrm{P}_{1\mathrm{dB}}}\xspace}
\newcommand{\lnagain}{\ensuremath{{G}_{\mathrm{rx}}}\xspace}
\newcommand{\papr}{\ensuremath{\mathrm{PAPR}}\xspace}
\newcommand{\adcbits}{\ensuremath{b}\xspace}
\newcommand{\adcbitslost}{\ensuremath{b_{\mathrm{lost}}}\xspace}
\newcommand{\adcdr}{\ensuremath{\mathcal{D}}\xspace}
\newcommand{\Prxadc}{\ensuremath{P_{\mathrm{rx}}}\xspace}

\newcommand{\powernoise}{\ensuremath{P_{\mathrm{noise}}}\xspace}
\newcommand{\powerdes}{\ensuremath{P_{\mathrm{des}}}\xspace}
\newcommand{\powersi}{\ensuremath{P_{\mathrm{SI}}}\xspace}
\newcommand{\powerquant}{\ensuremath{P_{\mathrm{quant}}}\xspace}

==> par-notation-v2.tex <==
% We use the following notation and conventions. 
We use one-indexing unless otherwise specified.
We represent matrices with bold uppercase, $\mat{A}$. 
We represent column vectors with bold lowercase, $\vec{a}$. 
We represent sets with script lettering, $\set{A}$.
We represent scalars with standard lowercase, $a$, standard uppercase, $A$, and sometimes script lettering, $\mathcal{A}$, for important quantities.
We define $\j = \sqrt{-1}$.
% We use $(\cdot)$\trans, $(\cdot)$\ctrans, and \frobenius{\cdot} to represent matrix transpose, conjugate transpose, and Frobenius norm, respectively. 
We use $(\cdot)\trans$ and $(\cdot)\ctrans$ to represent matrix transpose and conjugate transpose, respectively.
% We use $\normtwo{\cdot}$, $\normfro{\cdot}$, and $\ev{\cdot}$ as the $\ell_{2}$ vector norm, Frobenius norm, and expectation, respectively.
% An induced matrix norm is defined as $\norm{\mat{A}} = \max_{\vec{x}} \norm{\mat{A}\vec{x}} / \norm{\vec{x}}$ where $\norm{\cdot}$ is some vector norm.
% We use $\trace{\mat{A}}$, $\vectorize{\mat{A}}$, $\bars{\mat{A}}$, and $\ev{\cdot}$ to represent the trace of \mat{A}, the column vectorization of \mat{A}, the determinant of \mat{A}, and expectation, respectively. 
We use $\trace{\mat{A}}$ and $\bars{\mat{A}}$ to represent the trace of \mat{A} and the determinant of \mat{A}, respectively. 
% We overload $\diag{\mat{A}}$ and $\diag{\vec{a}}$ to represent a vector of the main diagonal elements of $\mat{A}$ and a square diagonal matrix with the elements of \vec{a} on the main diagonal, respectively.
We use $\diag{\mat{A}}$ to represent a vector of the main diagonal elements of $\mat{A}$.
% ; by this convention, $\diag{\diag{\mA}}$ represents a diagonal matrix whose diagonal elements are the diagonal elements of $\mA$.
% We use $\kron$ and $\had$ to represent the Kronecker and Hadamard products, respectively.
We use $\card{\set{A}}$ to represent the cardinality of a set $\set{A}$.
% We use $\svmax{\mA}$ to denote the maximum singular value and maximum eigenvalue of \mat{A}, respectively.
We use $\left[\mat{A}\right]_{i,j}$ to denote the element in the $i$-th row and $j$-th column of \mat{A}. 
We use $\left[\mat{A}\right]_{i,:}$ and $\left[\mat{A}\right]_{:,j}$ to denote the $i$-th row and $j$-th column of \mat{A}, respectively. 
% We use $\mI$ as an identity matrix.
% We use $(\cdot)\todB$ to represent a quantity in unit of \gls{db}. 
% We use $\todB{x} = 10 \log_{10}(x)$ to represent $x$ in units of \glspl{db}.
% We use $\todBm{x}$ to represent $x$ in units of \glspl{dbm}.
% We use $\complexpow{m}{n}$ to represent the set of all $m\times n$ matrices with complex entries.
% Finally, we use \eyevec{N} to denote an $N$-element column vector of ones and \eyemat{N} to denote an $N \times N$ identity matrix.
We use $\cgauss{\vec{m}}{\mat{R}}$ as a multivariate circularly symmetric complex Normal distribution with mean $\vec{m}$ and covariance matrix $\mat{R}$.
% We often use set-builder notation when defining sets.
% We use $\binom{n}{k} = \frac{n!}{k!(n-k)!}$ to denote the $n$-choose-$k$ binomial coefficient.
% We use $\land$ as a logical AND operation.
% We distinguish matrices and vectors in the time domain as $\mat{A},\vec{a}$ and in the frequency domain as $\matfd{A},\vecfd{a}$.
% We use the term ``beamformer'' most often to refer to a single column (rather than matrix) of beamforming weights.

==> par-notation.tex <==
We use the following notation and conventions. 
We use one-indexing unless otherwise specified.
We represent matrices with bold uppercase, $\mat{A}$. 
We represent column vectors with bold lowercase, $\vec{a}$. 
We represent sets with script lettering, $\set{A}$.
We represent scalars with standard lowercase, $a$, standard uppercase, $A$, and sometimes script lettering, $\mathcal{A}$, for important quantities.
We define $\j = \sqrt{-1}$.
% We use $(\cdot)$\trans, $(\cdot)$\ctrans, and \frobenius{\cdot} to represent matrix transpose, conjugate transpose, and Frobenius norm, respectively. 
We use $(\cdot)\trans$, $(\cdot)\ctrans$, and $(\cdot)\conj$ to represent matrix transpose, conjugate transpose, and conjugate, respectively.
We use $\normone{\cdot}$, $\normtwo{\cdot}$, $\norminf{\cdot}$, and $\normfro{\cdot}$ as the $\ell_{1}$, $\ell_{2}$, $\ell_{\infty}$, and Frobenius vector norms and induced matrix norms, respectively.
% An induced matrix norm is defined as $\norm{\mat{A}} = \max_{\vec{x}} \norm{\mat{A}\vec{x}} / \norm{\vec{x}}$ where $\norm{\cdot}$ is some vector norm.
We use $\trace{\mat{A}}$, $\vectorize{\mat{A}}$, $\bars{\mat{A}}$, and $\ev{\cdot}$ to represent the trace of \mat{A}, the column vectorization of \mat{A}, the determinant of \mat{A}, and expectation, respectively. 
We overload $\diag{\mat{A}}$ and $\diag{\vec{a}}$ to represent a vector of the main diagonal elements of $\mat{A}$ and a square diagonal matrix with the elements of \vec{a} on the main diagonal, respectively; by this convention, $\diag{\diag{\mA}}$ represents a diagonal matrix whose diagonal elements are the diagonal elements of $\mA$.
% We use $\kron$ and $\had$ to represent the Kronecker and Hadamard products, respectively.
We use $\card{\set{A}}$ to represent the cardinality of a set $\set{A}$.
We use $\svmax{\mA}$ and $\evmax{\mA}$ to denote the maximum singular value and maximum eigenvalue of \mat{A}, respectively.
We use $\left[\mat{A}\right]_{i,j}$ to denote the element in the $i$th row and $j$th column of \mat{A}. 
We use $\left[\mat{A}\right]_{i,:}$ and $\left[\mat{A}\right]_{:,j}$ to denote the $i$th row and $j$th column of \mat{A}, respectively. 
We use $\mI$ as an identity matrix.
% We use $(\cdot)\todB$ to represent a quantity in unit of \gls{db}. 
We use $\todB{x} = 10 \log_{10}(x)$ to represent $x$ in units of \glspl{db}.
We use $\todBm{x}$ to represent $x$ in units of \glspl{dbm}.
We use $\complexpow{m}{n}$ to represent the set of all $m\times n$ matrices with complex entries.
% Finally, we use \eyevec{N} to denote an $N$-element column vector of ones and \eyemat{N} to denote an $N \times N$ identity matrix.
We use $\cgauss{\vec{m}}{\mat{R}}$ as a multivariate circularly symmetric complex Normal distribution with mean $\vec{m}$ and covariance matrix $\mat{R}$.
We often use set-builder notation when defining sets.
We use $\binom{n}{k} = \frac{n!}{k!(n-k)!}$ to denote the $n$-choose-$k$ binomial coefficient.
% We use $\land$ as a logical AND operation.
% We distinguish matrices and vectors in the time domain as $\mat{A},\vec{a}$ and in the frequency domain as $\matfd{A},\vecfd{a}$.
% We use the term ``beamformer'' most often to refer to a single column (rather than matrix) of beamforming weights.

==> sec-algorithm.tex <==
\section{Algorithm} \label{eq:sec-algorithm}

\subsection{Solving our Problem}
To solve this, we formulate an optimization problem as follows.
First, let us express our constraints as
\begin{gather}
\mathcal{C}_{\mathrm{pow}}\parens{\prebb\node{i}} \triangleq \brackets{\normfro{\prebb\node{i}}^2 - 1}^+ \\
\mathcal{C}_{\mathrm{LNA}}\parens{\prebb\node{i}} \triangleq \brackets{\frac{1}{\Ns\node{i}} \pnorm{\infty}{\sqrt{\Ptxwatts\node{i}} G_{ii} \channel_{ii} \prerf\node{i} \prebb\node{i}}^2 - \powersimaxlna}^+ \\
\mathcal{C}_{\mathrm{ADC}}\parens{\prebb\node{i}} \triangleq \brackets{\frac{1}{\Ns\node{i}} \pnorm{\infty}{\sqrt{\Ptxwatts\node{i}} G_{ii} \comrf\ctransnode{i} \channel_{ii} \prerf\node{i} \prebb\node{i}}^2 - \powersimaxadc}^+
\end{gather}
where 
\begin{align}
\brackets{x}^+ = \max\braces{0,x}
\end{align}
We then transform it to a minimization problem and augment the original objective with our constraints as penalty terms as follows.
\begin{align}
\min_{\prebb\node{i}} \ & 
- \mathcal{I}_{ij}\parens{\prebb\node{i}} 
+ \lambda_{\mathrm{pow}} \cdot \mathcal{C}_{\mathrm{pow}}\parens{\prebb\node{i}} 
+ \lambda_{\mathrm{LNA}} \cdot \mathcal{C}_{\mathrm{LNA}}\parens{\prebb\node{i}} 
+ \lambda_{\mathrm{ADC}} \cdot \mathcal{C}_{\mathrm{ADC}}\parens{\prebb\node{i}}
\label{eq:unconstrained-augmented}
\end{align}
where $\lambda_{\mathrm{pow}}, \lambda_{\mathrm{LNA}}, \lambda_{\mathrm{ADC}} \geq 0$ are penalty multipliers.
Solving this problem with properly selected penalty multipliers would be equivalent to solving the original constrained problem.
Finding the appropriate choices for $\lambda_{\mathrm{pow}}, \lambda_{\mathrm{LNA}}, \lambda_{\mathrm{ADC}}$ is generally difficult.
One option is to solve \eqref{eq:unconstrained-augmented} at each point over a three dimensional search for $\lambda_{\mathrm{pow}}, \lambda_{\mathrm{LNA}}, \lambda_{\mathrm{ADC}}$.
To reduce this, we introduce a fourth penalty term $\nu$ and rewrite the problem as
\begin{align}
\min_{\prebb\node{i}} \ & 
- \mathcal{I}_{ij}\parens{\prebb\node{i}} 
+ \nu \brackets{\lambda_{\mathrm{pow}} \cdot \mathcal{C}_{\mathrm{pow}}\parens{\prebb\node{i}} 
	+ \lambda_{\mathrm{LNA}} \cdot \mathcal{C}_{\mathrm{LNA}}\parens{\prebb\node{i}} 
	+ \lambda_{\mathrm{ADC}} \cdot \mathcal{C}_{\mathrm{ADC}}\parens{\prebb\node{i}}}
\label{eq:unconstrained-augmented-2}
\end{align}
and fix $\lambda_{\mathrm{pow}}, \lambda_{\mathrm{LNA}}, \lambda_{\mathrm{ADC}}$ as follows
\begin{align}
\lambda_{\mathrm{pow}} &= 1 \\
\lambda_{\mathrm{LNA}} &= \frac{1}{\powersimaxlna} \\
\lambda_{\mathrm{ADC}} &= \frac{1}{\powersimaxadc}
\end{align}
which approximately weights the three constraints equally and allows us to abstract our three-dimensional search to a one-dimensional search over $\nu$.
We search for $\nu$ using bisection, where $\Nnu$ is the number of bisection steps and $\numin$ and $\numax$ are the minimum and maximum values of $\nu$ our search covers, respectively.

Given that a practical implementation of our solver will be limited in precision (e.g., due to machine precision), we introduce $\epspow$, $\epslna$, and $\epsadc$ as tolerances associated with meeting each of our constraints.
By introducing these tolerances, our algorithm will naturally produce a solution that does not satisfy our constraints.
To account for this, we apply a final power projection to ensure all three constraints are met.
We begin by calculating the three scalars
\begin{gather}
g_{\mathrm{pow}} = \sqrt{\frac{1}{\normfro{\prebb\node{i}}^2}} \\
g_{\mathrm{LNA}} = \sqrt{\frac{\powersimaxlna}{\frac{1}{\Ns\node{i}} \pnorm{\infty}{\sqrt{\Ptxwatts\node{i}} G_{ii} \channel_{ii} \prerf\node{i} \prebb\node{i}}^2}} \\
g_{\mathrm{ADC}} = \sqrt{\frac{\powersimaxadc}{\frac{1}{\Ns\node{i}} \pnorm{\infty}{\sqrt{\Ptxwatts\node{i}} G_{ii} \comrf\ctransnode{i} \channel_{ii} \prerf\node{i} \prebb\node{i}}^2}}
\end{gather}
Then, choosing the minimum of these three yields
\begin{gather}
g_{\mathrm{proj}} = \min \braces{g_{\mathrm{pow}} , g_{\mathrm{LNA}} , g_{\mathrm{ADC}} }
\end{gather}
which we apply as
\begin{align}
\prebb\node{i} = \prebb\node{i} \times g_{\mathrm{proj}}
\end{align}
% After the algorithm runs, we merely project to ensure the three constraints are met.

An optimality condition is at least one of the three constraints is tight since more power could be supplied to increase the mutual information.


\input{alg/algorithm-v1.tex}

\subsection{Accelerating our Optimization}

Let $\mat{A} \in \setmatrixcomplex{m}{n}$. We have the following matrix norm inequalities.
\begin{gather}
\normtwo{\mat{A}} \leq \normfro{\mathbf{A}} \leq \sqrt{n} \normtwo{\mat{A}} \\
\frac{1}{\sqrt{n}} \norminf{\mat{A}} \leq \normtwo{\mathbf{A}} \leq \sqrt{m} \norminf{\mat{A}}
\end{gather}
Together, this allows us to write
\begin{gather}
\normfro{\mathbf{A}} \leq \sqrt{n} \normtwo{\mat{A}} \leq \sqrt{mn} \norminf{\mat{A}} \\
\norminf{\mathbf{A}} \leq \sqrt{n} \normtwo{\mat{A}} \leq \sqrt{n} \normfro{\mat{A}},
\end{gather}

We note that the following holds
\begin{align}
\frac{1}{\Ns\node{i}} \norminf{\sqrt{\Ptxwatts\node{i}} G_{ii} \channel_{ii} \prerf\node{i} \prebb\node{i}}^2 
&\leq \frac{1}{\Ns\node{i}} \norminf{\sqrt{\Ptxwatts\node{i}} G_{ii} \channel_{ii} \prerf\node{i}}^2 \cdot \norminf{\prebb\node{i}}^2 \\
&\leq \frac{1}{\Ns\node{i}} \norminf{\sqrt{\Ptxwatts\node{i}} G_{ii} \channel_{ii} \prerf\node{i}}^2 \cdot \Ns\node{i} \normfro{\prebb\node{i}}^2 \\
&\leq \norminf{\sqrt{\Ptxwatts\node{i}} G_{ii} \channel_{ii} \prerf\node{i}}^2
\end{align}

This allows us to check if the \lna constraint needs to be included in the optimization for a given choice of $\prerf\node{i}$.
Explicitly, if the following holds for a candidate having $\prerf\node{i}$
\begin{align}
\norminf{\sqrt{\Ptxwatts\node{i}} G_{ii} \channel_{ii} \prerf\node{i}}^2 \leq \powersimaxlna \label{eq:accelerate-criteria-lna}
\end{align}
we can rewrite our problem as
\begin{subequations} \label{eq:problem-inner-v2}
	\begin{align}
	\max_{\prebb\node{i}} \ & \mathcal{I}_{ij}\parens{\prebb\node{i}} \label{eq:problem-inner-v2-obj} \\
	\st \ 
	& \frobeniustwo{\prebb\node{i}} \leq 1 \label{eq:problem-inner-v2-power}\\
	& \frac{1}{\Ns\node{i}} \pnorm{\infty}{\sqrt{\Ptxwatts\node{i}} G_{ii} \comrf\ctransnode{i} \channel_{ii} \prerf\node{i} \prebb\node{i}}^2 \leq \powersimaxadc  
	\end{align}
\end{subequations}
since any feasible $\prebb\node{i}$ will simultaneously satisfy our \lna constraint by satisfying \eqref{eq:problem-inner-v2-power}.

In a similar fashion, we can extend this concept to the \adc constraint.
\begin{align}
\frac{1}{\Ns\node{i}} \norminf{\sqrt{\Ptxwatts\node{i}} G_{ii} \comrf\ctransnode{i} \channel_{ii} \prerf\node{i} \prebb\node{i}}^2 
&\leq \frac{1}{\Ns\node{i}} \norminf{\sqrt{\Ptxwatts\node{i}} G_{ii} \comrf\ctransnode{i} \channel_{ii} \prerf\node{i}}^2 \cdot \norminf{\prebb\node{i}}^2 \\
&\leq \frac{1}{\Ns\node{i}} \norminf{\sqrt{\Ptxwatts\node{i}} G_{ii} \comrf\ctransnode{i} \channel_{ii} \prerf\node{i}}^2 \cdot \Ns\node{i} \normfro{\prebb\node{i}}^2 \\
&\leq \norminf{\sqrt{\Ptxwatts\node{i}} G_{ii} \comrf\ctransnode{i} \channel_{ii} \prerf\node{i}}^2
\end{align}
When considering a choice of $\prerf\node{i}$ and $\comrf\node{i}$, if the following holds
\begin{align}
\norminf{\sqrt{\Ptxwatts\node{i}} G_{ii} \comrf\ctransnode{i} \channel_{ii} \prerf\node{i}}^2 \leq \powersimaxadc \label{eq:accelerate-criteria-adc}
\end{align}
and \eqref{eq:accelerate-criteria-lna} does not, we can write our problem as
\begin{subequations} \label{eq:problem-inner-v3}
	\begin{align}
	\max_{\prebb\node{i}} \ & \mathcal{I}_{ij}\parens{\prebb\node{i}} \label{eq:problem-inner-v3-obj} \\
	\st \ 
	& \frobeniustwo{\prebb\node{i}} \leq 1 \\
	& \frac{1}{\Ns\node{i}} \pnorm{\infty}{\sqrt{\Ptxwatts\node{i}} G_{ii} \channel_{ii} \prerf\node{i} \prebb\node{i}}^2 \leq \powersimaxlna
	\end{align}
\end{subequations}

When both \eqref{eq:accelerate-criteria-lna} and \eqref{eq:accelerate-criteria-adc} hold, our problem reduces merely to
\begin{subequations} \label{eq:problem-inner-v4}
	\begin{align}
	\max_{\prebb\node{i}} \ & \mathcal{I}_{ij}\parens{\prebb\node{i}} \label{eq:problem-inner-v4-obj} \\
	\st \ 
	& \frobeniustwo{\prebb\node{i}} \leq 1
	\end{align}
\end{subequations}
whose solution is the known eigen-based, water-filled precoder.

\subsection{Further Acceleration}
Since the aforementioned accelerations depend on the \rf candidates, candidate acquisition may require its candidates to satisfy \eqref{eq:accelerate-criteria-lna} and \eqref{eq:accelerate-criteria-adc} to reduce the computational overhead associated with solving \eqref{eq:problem-inner} for each candidate pair.

Having knowledge of $\channel_{ii}$ and the codebooks from which $\prerf\node{i}$ and $\comrf\node{i}$ are drawn, the full-duplex device can compute \eqref{eq:accelerate-criteria-lna} and \eqref{eq:accelerate-criteria-adc} over all possible pairs of $\prerf\node{i}$ and $\comrf\node{i}$. 
Pairs satisfying \eqref{eq:accelerate-criteria-lna} and/or \eqref{eq:accelerate-criteria-lna} will be considered as possible selections and those that do not can be discarded.
Of course, this sacrifices optimality, but greatly reduces the computational overhead of our design.
While this must be repeated for each realization of $\channel_{ii}$, this acceleration may take into account the long-term statistics of $\channel_{ii}$ to build our set of possible candidates.

==> sec-keywords.tex <==
\begin{keywords}
Millimeter-wave
\end{keywords}

==> sec-peer-review-title.tex <==
% For peer review papers, you can put extra information on the cover
% page as needed:
% \ifCLASSOPTIONpeerreview
% \begin{center} \bfseries EDICS Category: 3-BBND \end{center}
% \fi
%
% For peerreview papers, this IEEEtran command inserts a page break and
% creates the second title. It will be ignored for other modes.
\IEEEpeerreviewmaketitle
